Cyber-All-Intel: An AI for Security related Threat Intelligence

Keeping up with threat intelligence is a must for a security analyst today. There is a volume of information present in `the wild' that affects an organization. We need to develop an artificial intelligence system that scours the intelligence sources, to keep the analyst updated about various threats that pose a risk to her organization. A security analyst who is better `tapped in' can be more effective. In this paper we present, Cyber-All-Intel an artificial intelligence system to aid a security analyst. It is a system for knowledge extraction, representation and analytics in an end-to-end pipeline grounded in the cybersecurity informatics domain. It uses multiple knowledge representations like, vector spaces and knowledge graphs in a 'VKG structure' to store incoming intelligence. The system also uses neural network models to pro-actively improve its knowledge. We have also created a query engine and an alert system that can be used by an analyst to find actionable cybersecurity insights.

==> Sections/03_model_FULL.tex <==
In this section we describe our VKG structure, which leverages both vector spaces and knowledge graphs to create a new representation for relations and entities of interest present in text. In the VKG structure, an entity is represented as a node in a knowledge graph and is linked to its representation in a vector space. Figure \ref{fig:ex} gives an example of the VKG structure where entity nodes are linked to each other using explicit relations as in a knowledge graph and are also linked to their word embeddings in a vector space. The VKG structure enables an application to reason over the knowledge graph portion of the structure and also run computations on the vector space part. 

\begin{figure}[h]
\centering
\includegraphics[scale=0.18]{images/example.pdf}
\caption{An example of a VKG structure representing ``Tom has a pet Milo and Milo is a cat''.}
\label{fig:ex}
\end{figure}

The VKG structure enables us to specifically assert information present in the vector representation of concepts and entities using semantic relations, for example, in Figure \ref{fig:ex}; using the VKG structure we can explicitly assert that the vector representation of `Milo' and `Cat' are related like, $<Milo, isA, Cat>$. `Tom' and `Milo' are related with the relation, $<Tom, hasPet, Milo>$. The vector representation of `Milo' can be used to find other pets that are similar to it, but the explicit information that `Milo' is a `Cat' and it's `Tom' that has a pet named `Milo' can be accurately derived explicitly from the knowledge graph part. 

The VKG structure helps us unify knowledge graphs and vector representation of entities, and allows us to develop powerful inference methods that combine their complementary strengths.

The vector representation we use is based on the `Relational Concurrence Assumption' highlighted in \cite{mikolov2013distributed,mikolov2013efficient,collobert2011natural}. Word embeddings are able to capture different degrees of similarity between words. Mikolov et al. \cite{mikolov2013distributed,mikolov2013efficient} argue that embeddings can reproduce semantic and syntactic patterns using vector arithmetic. Patterns such as ``Man is to Woman as King is to Queen'' can be generated through algebraic operations on the vector representations of these words such that the vector representation of ``King'' - ``Man'' + ``Woman'' produces a result which is closest to the vector representation of ``Queen'' in the model. Such relationships can be generated for a range of semantic relations as well as syntactic relations. However, in spite of the fact that vector space models excel at determining similarity between two vectors they are severely constrained while creating complex dependency relations and other logic based operations that are a forte of various semantic web based applications \cite{davis1993knowledge,berners2001semantic}. 

Knowledge graphs, on the other hand, are able to use powerful reasoning techniques to infer and materialize facts as explicit knowledge. Those based on description logic representation frameworks like OWL, for example, can exploit axioms implicit in the graphs to compute logical relations like consistency, concept satisfiability, disjointness, and subsumption. As a result, they are generally much slower while handling operations like, ontology alignment, instance matching, and semantic search \cite{shvaiko2013ontology,JeanMary2009OntologyMW}.

The intuition behind our approach is that an entity's context from its immediate neighborhood, present as word embeddings, adds more information along with various relations present explicitly in a knowledge graph. Entity representation in vector space gives us information present in the immediate context of the place where they occur in the text and knowledge graphs give us explicit information that may or may not be present in the specific piece of text. Embeddings can help find similar nodes or words faster using neighborhood search algorithms and search space reductions. They also support partial matching techniques. Knowledge graphs provide many reasoning tools including query languages like SPARQL\footnote{\url{https://www.w3.org/TR/rdf-sparql-query/}}, rule languages like SWRL\footnote{\url{https://www.w3.org/Submission/SWRL/}}, and description logic reasoners.

Potential applications that will work on our VKG structure, need to be designed to take advantages provided by integrating vector space models with a knowledge graph. In a general efficient use-case for our VKG structure, `fast' top-k search should be done on the vector space part aided by the knowledge graph, and the `slow' reasoning based computations should be performed on just the knowledge graph part. An input query can be decomposed into sub-queries which run on respective parts of the VKG structure (see \ref{query}). We analogize this to thinking `fast' in vector space along with thinking `deeply' and `slowly' by using the knowledge graph. 

%\begin{figure}[h]
%\centering
%\includegraphics[scale=0.19]{images/domaininformation.pdf}
%\caption{Adding medical domain knowledge using the VKG structure.}
%\label{fig:domain}
%\end{figure}

\begin{figure*}[ht]
\centering
\includegraphics[scale=0.3]{images/cyberexample.pdf}
\caption{In the VKG structure for \textit{``Microsoft Internet Explorer allows remote attackers to execute arbitrary code or cause a denial of service (memory corruption) via a crafted web site, aka ``Internet Explorer Memory Corruption Vulnerability.''} the knowledge graph part asserted using UCO includes the information that a product `Microsoft Internet Explorer' has vulnerabilities `execute arbitrary code' and `denial of service' that can be exploited by `remote attackers' using the means `crafted web site'. The knowledge graph entities are linked to their vector embeddings using the relation `hasVector'.}
\label{fig:cyberexample}
\end{figure*}


By using the VKG structure, we link entity vector embeddings with their knowledge graph nodes. Domain specific knowledge graphs are built using a schema that is generally curated by domain experts. When we link the nodes and embeddings we can use the explicit information present in these ontologies to provide domain understanding to embeddings in vector space. Adding domain knowledge to vector embeddings can further improve various applications built upon the structure. The vector embeddings can be used to train machine learning models for various tasks. These machine learning models can use explicit assertions present in the knowledge graph part. This will also help in improving the quality of the results generated for various input queries discussed in Section \ref{query}.

%In another example from the medical domain (Figure \ref{fig:domain}) we use the VKG structure to state that the vector embedding of `skin' belongs to the class `Organ' which is a subclass of `Body Substance'. In a cybersecurity example (Figure \ref{fig:cyberexample}) from our Cyber-All-Intel system discussed in Section \ref{mysystem}, we explicitly state that `denial\_of\_service' is a vulnerability. Using the VKG structure we connect the fact that the vector embedding of `denial\_of\_service' is a vulnerability. 

In the example, (Figure \ref{fig:ex}) we can use the VKG structure to state that the vector embedding of `Milo' belongs to the class `Cat', which is a subclass of `Mammals' and so on. In a cybersecurity example (Figure \ref{fig:cyberexample}) from our Cyber-All-Intel system discussed in Section \ref{system}, we explicitly state that `denial\_of\_service' is a vulnerability. Using the VKG structure we connect the fact that the vector embedding of `denial\_of\_service' is a vulnerability.

Knowledge graph nodes in the VKG structure can be used to add information from other sources like DBpedia, YAGO, and Freebase. This helps integrate information that is not present in the input corpus. For example, in Figure \ref{fig:cyberexample} we can link using the `$owl:sameAs$' property `Microsoft\_Internet\_Explorer' to its DBpedia equivalent `dbp:Internet\_Explorer'. Asserting this relation adds information like Internet Explorer is a product from Microsoft. This information may not have been present in the input cybersecurity corpus but is present in DBpedia.

In the rest of this section, we will discuss populating the VKG structure (Section \ref{pop}), query processing on the structure (Section \ref{query}).%, and various use-cases (Section \ref{apps}). 

\subsection{Populating the VKG Structure} \label{pop}

In order to create the VKG structure, the structure population system requires as input, a text corpus. The aim of the system is to create the VKG structure for the concepts and entities present in the input corpus which requires us to create the knowledge graph and the vector parts separately and then linking the two. 

Various steps and technologies required are enumerated below. The Cyber-All-Intel system that uses the VKG structure to represent a textual corpus is described in Section \ref{system}.

\begin{enumerate}

\item \textit{Training vectors}: For the vector part of the VKG structure, we can generate entity embeddings using any of a number of vectorization algorithms. For text, many of these are based on the `Relational Concurrence Assumption' principle \cite{mikolov2013distributed,mikolov2013efficient,pennington2014glove,huang2012improving}. 

\item \textit{Creating semantic triples}:  An information extraction pipeline  extracts a knowledge graph from a collection of text documents.  The first step applies components from Stanford CoreNLP components \cite{manning2014stanford} trained to recognize entities and relations in the cybersecurity domain to produce a knowledge graph for each document.  The second step uses components from Kelvin \cite{finin2016hltcoe} to integrate the document-level graphs by performing cross-document co-reference, linking entities to reference knowledge bases like DBpedia, and drawing additional inferences.  The resulting knowledge graph is then materialized as an RDF graph.

\item \textit{Creating links between entity vectors and nodes}: We link knowledge graph nodes to their corresponding words in the vector space vocabulary using the $hasVector$ relationship as shown in Figure \ref{fig:ex}. Keeping the lexical tokens in the knowledge graph allows us to update vector embeddings as the underlining corpus changes and renders the vector model stale. This symbolic linking of the knowledge graph part and the vector part via the $hasVector$ relation is initiated after the RDF triples are generated. 

\end{enumerate}

The computational complexity to create the VKG structure can be derived form the steps mentioned above. These are detailed in extent literature \cite{mikolov2013efficient,finkel2005incorporating,angeli2015leveraging}. To create the vector space model the complexity is proportional to the word context window ($N$), vector dimensionality ($D$) and the hidden layer size ($H$)\footnote{Here we assume there is only 1 hidden layer}. To create the RDF triples, we use a named entity recognizer and relationship extractors where the complexity is proportional to the number of entity classes ($C$) and the set of relations ($R$). Computational complexity of the linking step depends on the vocabulary size of the corpus ($V$). So the computational complexity to create one structure:

\[ (N \times D \times H)+(C+R)+V \]

While creating the VKG structures for the Cyber-All-Intel system on cybersecurity corpus of vocabulary size 246,321, the RDF triple generation part $(C + R)$ took most of the time. For an application the vector model may need to be retrained after some time to account for new incoming data, so the $(N \times D \times H)$ part runs periodically (in the Cyber-All-Intel system once every two weeks). Complexity of the linking process $(V)$ can be improved using hashing, it will also improve the performance of the query processing engine described in Section \ref{query}.



==> Sections/03h_derived.tex <==
Another type of queries that are possible on the VKG structure are certain queries that build up on derived concepts. An example of the derive concept is the node `Int3482758232' in Figure \ref{fig:cyberexample}. The node is of the class \textit{intelligence} and points to a piece of information about a `execute\_arbitrary\_code' \& `denial\_of\_service' vulnerability in the product `Microsoft\_Internet\_Explorer' and its associated meta-data. The derived concept is completely dependent on the information present about its underlying defining concepts. These derived entities have meaning only in an abstract sense. A query to figure out how similar or different is one such derived concept motivates the need for their vector space representation based on various underlying concepts. Vector representation for derived concepts will enable scoring, indexing, entity weighting, analogical mapping, nearest / neighborhood search, etc. by utilizing the vector space; rather than being dependent on the knowledge graph for these tasks. Knowledge graphs on the other hand will provide a more robust way to differentiate between derived concepts and a method for an analyst to check the provenance of the information. 

An important property about these derived concepts is that they are created during the knowledge population stage and their embeddings are not generated using the vector creation process as they are generally not present in the text corpus. 

In order to create embeddings for these concepts we need to keep some requirements in mind: 
\begin{enumerate} 
\item The primary requirement is that similar derived concepts should be closer together. %WORD. For memory and computational constraints we wish to create embeddings for the derived concepts in the same vector space as the underlying concepts.  

\item Adding out-of-space details and meta-data to the embeddings will require vector space extensions. An example, of such meta-data is time. Time may not have been included in the vector space created for the underlying embeddings, and extra dimensions will need to be added to incorporate time for derived concept embeddings. 

\item Another requirement for out embeddings is that updates to vector embeddings for underlying concepts trickle fast to the vector representation for derived concepts. This requirement is critical in our generation scheme as the vectors for the derived concepts are dependent on the underlying concepts, and time critical updates to these embeddings should be factored in the derived embeddings. 

\end{enumerate}
%The motivation for creating these derived vectors comes from  , cybersecurity intelligence events news, 
In order to create vector embeddings for these derived entities we start with vector representation of the underlying concepts. Let the set of underlying concept vectors be $V$.

\[ V = \{v_{1},\, v_{2},\, v_{3},\, v_{4},\, v_{5},\, ...\} \]

Here, $v_{1}, v_{2}, v_{3}, ...$ represent the vectors for the underlying concepts in a $d$ dimensional space. Also, $w$ represents the set of scalar weights assigned to these vectors. These scalar weights can be used to assign different weight-age to the underlying concepts. 

\[ w = \{w_{1},\, w_{2},\, w_{3},\, w_{4},\, w_{5},\, ...\} \]
\[ V_{w} = wV \]
\[ V_{w} = \{w_{1}v_{1},\, w_{2}v_{2},\, w_{3}v_{3},\, w_{4}v_{4},\, ...  \} \]

So the task is to create the vector $v_{d}$ using the set of vectors $V_{w}$. 

So as to do these computations fast and more importantly, so as to ensure that the changes in the vector embeddings for the underlining concepts propagate to these derived embeddings we use a variety of mathematical methods to generate these embeddings like, addition \eqref{addivec}, hadamard \eqref{hada}. 

\[ v_{d} = w_{1}v_{1} + w_{2}v_{2} + w_{3}v_{3} + w_{4}v_{4} + ...   \tag{a} \label{addivec}\]
\[ v_{d} = w_{1}v_{1} \odot w_{2}v_{2} \odot w_{3}v_{3} \odot w_{4}v_{4} \odot ...  \tag{b}\label{hada}\]

We discuss and evaluate the results obtained using both these methods in Section \ref{eval}. These derived vectors are then used in the applications discussed in Section \ref{appl}. 
%lack of training data so no deep learning based 

%some generated test data to evaluate

%however in our case 

%we found that addition gave the best results. we believe that this was because 

%Using vector addition to create vector space representation of these knowledge graph entities. 

%FIGURE

==> Sections/04_eval.tex <==
\section{Evaluations}\label{eval}
\subsection{Query Processing System}
Using the above mentioned data and annotation test sets we evaluate the different parts of our VKG structure and the query processing engine. In Section \ref{query}, we describe our query processing engine and its three query commands: $search$, $list$, and $infer$. Here we evaluate $search$ and $list$ query but not the $infer$ queries as they depend on the reasoning logic provided in the ontology and can vary with application.

\textit{Evaluation tasks:} We evaluate $search$ by comparing the performance of three models: vector embeddings, knowledge graph, and VKG search. Queries of type $list$ can only be run on the knowledge graph part of the VKG structure as there is no declarative information present in the embeddings. To evaluate the $list$ query we evaluate the quality of triples generated in the knowledge graph. We also evaluate the vector space and knowledge graph linking, as good quality linking is necessary for various operations on the VKG structure.

\subsubsection{Evaluating the $search$ query}

An input query to the VKG structure to find similar concepts can either run on the vector space using various neighborhood search algorithms \cite{gionis1999similarity,Kuzi:2016:QEU:2983323.2983876} or the knowledge graph using ontology matching, ontology alignment, schema matching, instance matching, similarity search, etc. \cite{shvaiko2013ontology,DeVirgilio:2013:SMA:2457317.2457352,zheng2016semantic}. We evaluate claims in Section \ref{query} that we get better and faster results using the vector space instead of the knowledge graph for similarity computations. We also show that knowledge graph aided vector spaces (VKG search) provide the best results when compared to vector spaces and knowledge graphs alone.  

%In order to evaluate the $search$ query we evaluate the vector space part and compare searching on the vector space to instance matching on the knowledge graph. 

\textit{Evaluating the Vector Space Models:} To evaluate the vector embeddings part of the VKG structure we used the `similar' sets created by the annotators. We trained various vector space models with vector dimension, 500, 1000, 1500, 1800, 2500 and term frequency, 1, 2, 5, 8, 10. Increasing the value of dimensionality and decreasing the term frequency almost exponentially increases the time to generate the vector space models. We first find the combination of parameters for which the Mean Average Precision (MAP) is highest, so as to use it in comparing the performance of vector space models with knowledge graphs and graph aided vectors in the VKG structure, in finding similar vulnerabilities, attacks, and products. For the 56 similar groups the vector model with dimensionality of 1500 and term frequency 2, had the highest MAP of 0.69 (Figure \ref{fig:map}). Models with higher dimensions and word frequency performed better.

\begin{figure}[h]
\centering
\includegraphics[scale=0.25]{images/MAP.png}
\caption{Mean Average Precision for different dimensions and word frequency. Models with higher dimensions and word frequency performed better.}
\label{fig:map}
\end{figure}

\textit{Comparing Vector Space Models and Knowledge Graphs:}  To compare the performance of the $search$ query over vector space and its counterpart from the knowledge graph side we used the vector embedding model with dimensionality of 1500 and term frequency 2. To compute instance matching on knowledge graphs, we used an implementation of ASMOV (Automated Semantic Matching of Ontologies with Verification) \cite{JeanMary2009OntologyMW}. On computing the MAP for both vector embeddings and the knowledge graphs we found that embeddings constantly outperformed the knowledge graphs. Figure \ref{fig:map2}, shows that the MAP value for vector embeddings was higher 47 times out of 56 similarity groups considered. The knowledge graph performed significantly bad for vulnerabilities and attacks as the structural schema for both attacks and vulnerabilities was quite dense with high number of edges to different entities. This significantly affected the performance of schema matching. We also found that computing $search$ queries was faster on vector embeddings as compared to knowledge graphs. Neighborhood search on vector spaces was empirically 11 times faster in our experiments compared to knowledge graphs.

\begin{figure}[h]
\centering
\includegraphics[scale=0.17]{images/mapvkg.png}
\caption{The number of times the MAP score was higher for the two knowledge representation techniques for the 56 similar groups. Vector embeddings performed better than knowledge graphs. Embeddings performed better in 8 attacks, 26 products, and 13 vulnerabilities.}
\label{fig:map2}
\end{figure}

\textit{Comparing Vector Space Models and VKG Search:} To test the advantages of our VKG structure we evaluate the VKG search (see Section \ref{query}) against the vector space model. The VKG search on vector space achieved a MAP of 0.8, which was significantly better than the MAP score (0.69) achieved by using just the vector model. The reason for higher quality results obtained by using the VKG search is due to the fact that we can filter out entities by using class type declarations present in the knowledge graph.

\begin{table}[h]
\centering
    \begin{tabular}{|c|c|c|c|}
    \hline
    \textbf{Model} & Graphs & Vectors & VKG Search \\ \hline
    \textbf{MAP}   & 0.43   & 0.69    & 0.80         \\ \hline
    \end{tabular}
    \caption{Best Mean Average Precision for knowledge graphs, vector space models, and VKG structure.}
\end{table}

\subsubsection{Evaluating the $list$ query}

Since the declarative assertions are made in the VKG's knowledge graph, to evaluate the $list$ query we evaluate the quality of the knowledge graph part. The $list$ query can not be executed on the vector space as there is no declarative information in embeddings. 

To check the quality of the knowledge graph triples generated from the raw text we asked the same set of annotators to manually evaluate the triples created and compare them with the original text. The annotators were given three options, correct, partially correct, and wrong. From 250 randomly selected text samples from the cybersecurity data, the annotators agreed that 83\% were marked correct, 9\% were partially correct, and 8\% were marked wrong.

\subsubsection{Evaluating Vector and Graph linking} To check the quality of the linkages created in the VKG structure, we again asked the annotators to review various nodes in the triples and check if they were linked to the right vocabulary word from the vector models generated. On evaluating 250 randomly selected triples the annotators found 97\% of them were linked correctly. This high accuracy can be attributed to the fact that both knowledge graphs and the vector space models had the same underlying corpus vocabulary. 

\subsection{Recommendation and Alerts}



==> Sections/05_concfuture.tex <==
\section{Conclusion \& Future Work}
\label{conc}

We also demonstrated the VKG structure and the query processing engine by developing a system called \textit{Cyber-All-Intel} for knowledge extraction, representation and querying in an end-to-end pipeline grounded in the cybersecurity informatics domain. The system creates a cybersecurity corpus by collecting threat and vulnerability intelligence from various textual sources like, national vulnerability databases, dark web vulnerability markets, social networks, blogs, etc. which are represented as instances of our VKG structure. We use the system to answer complex cybersecurity informatics queries. 

Vector space models and knowledge graph both have some form of information loss, vector embeddings tend to lose the declarative nature of information, but are ideal for similarity computation, indexing, scoring, neighborhood search, etc. Knowledge graphs, on the other hand, are good for asserting declarative information and have well developed reasoning techniques, perform slower. Together, they can both add value to each other. Using a hybrid of the two we can use the knowledge graph's declarative powers to explicitly state relations between various embeddings in a vector space. For example, we can assert in a knowledge graph, the information that `an adult mouse has 16 teeth' which is tough to do in a vector space. On the other hand we can use the embeddings to figure out entities similar to `Arctic Tern' and use the knowledge graph to improve the quality of our results, by understanding that the query pertains to various bird species. 

In this paper, we described the design and implementation of a VKG structure which is part vector embeddings and part knowledge graph. We discussed a method to create the VKG structure and built a query processing engine that decomposes an input query to sub-queries with commands $search$, $list$, and $infer$. We showed that queries of the type $search$ should run on the vector part of the VKG structure and the results should be improved with the aid of knowledge graph assertions. We call this technique VKG search. $list$ and $infer$ run on the knowledge graph part to take advantage of the robust reasoning capabilities. Using the VKG structure, we can efficiently answer those queries which are not handled by vector embeddings or knowledge graphs alone. In our future work, we plan to add more types of commands and queries that can be processed on our VKG structure. We would also like to build more use-cases and applications on the VKG structure.
